Minimizing the Effect of Noise and Limited Dataset Size in Image Classification Using Depth Estimation as an Auxiliary Task with Deep Multitask Learning

Generalizability is the ultimate goal of Machine Learning (ML) image classifiers, for which noise and limited dataset size are among the major concerns. We tackle these challenges through utilizing the framework of deep Multitask Learning (dMTL) and incorporating image depth estimation as an auxiliary task. On a customized and depth-augmented derivation of the MNIST dataset, we show a) multitask loss functions are the most effective approach of implementing dMTL, b) limited dataset size primarily contributes to classification inaccuracy, and c) depth estimation is mostly impacted by noise. In order to further validate the results, we manually labeled the NYU Depth V2 dataset for scene classification tasks. As a contribution to the field, we have made the data in python native format publicly available as an open-source dataset and provided the scene labels. Our experiments on MNIST and NYU-Depth-V2 show dMTL improves generalizability of the classifiers when the dataset is noisy and the number of examples is limited.

==> bk.tex <==
\usepackage{comment}
\begin{comment}
TO BE REMOVED:


\begin{abstract}
  Noise and dataset size are two bold obstacles of Machine Learning (ML) models. Multitask Learning, on the other hand, is a framework in which numerous classification and regression scenarios can be handled. In our experiments, we develop a deep Multitask Learning (dMTL) network to execute image classification using depth estimation as an auxiliary task and apply that to multiple noisy and limited size MNIST \cite{LeCun2010MNIST} based datasets and demonstrate improvements in final results.\\
  \\
  \textbf{Keywords:} depth estimation, multitask learning, classification

\end{abstract}


\section{Introduction}

Machine Learning (ML) models, specifically Convolutional Neural Networks (CNN), are proven to be promising in different fields and contexts such as Medical Imaging, Gaming, Real Estate, and transportation. Nonetheless, their performance and generalization are conditioned on their access to a large amount of standardized and preprocessed annotated datasets. Aggregating labeled, clean, and abundant data examples is not a straightforward task if feasible. Hence, our goal is to decrease the sensitivity of the performance of CNNs to dataset size and noise. To do so, we create multiple customized datasets based on MNIST ~\cite{LeCun2010MNIST} and utilize deep Multitask Learning (dMTL) to perform our classification and depth estimation tasks.

\subsection{Multitask Learning}

The concept of dMTL is about performing multiple tasks simultaneously. The method of sharing parameters in dMTL, which is either hard \cite{Baxter1997Bayesian/Information} or soft \cite{Duong2015Low}, determines how the model is optimized for multiple learning tasks at hand \cite{Girshick2015Fast}. Even if the ultimate goal is to do a single task, dMTL can significantly improve performance for the specific task if the main task is augmented with other tasks (i.e., auxiliary tasks) \cite{Baxter1997Bayesian/Information}. dMTL leads to a better generalization of the model through introducing an inductive bias based on the comprehensive information in the image \cite{Ruder2017Overview}.

Considering our scenario and building upon the prior research on multitask learning, we regard depth estimation and classification as entangled tasks. We examine the effect of noise and dataset size on them and we form a dMTL setting to improve their performance effectively.

\section{An Overview on Depth Estimation Methods}
There are two main approaches for depth estimation; unsupervised and supervised. In unsupervised methods, stereo images are utilized to infer the 3D structure of the scene. In supervised methods, on the other hand, the model is trained on existing depth maps. Following is a review on both unsupervised and supervised approaches along with new experiments on depth estimation and image classification tasks using deep Multitask Learning (dMTL).

\subsection{Unsupervised Approaches}
Using unsupervised learning methods for depth estimation requires information from multiple images of a scene. These methods enable single image depth estimation without the need for the ground truth depth information. Since acquiring depth information for large amount of data is not always feasible, these approaches introduce an alternative solution to mitigate the limitations of obtaining ground truth depth labels.

\begin{itemize}
  \item \textbf{Unsupervised monocular depth estimation with left-right consistency:}\\
Godard et al. \cite{Godard2017Unsupervised} employ the left and right images of a view obtained from a binocular stereo footage in the training phase and only use images from one view in inference. By training the network with an image reconstruction loss and exploiting epipolar geometry constraints, disparity images are generated. The idea is to find the function that can reconstruct one side of a pair of binocular images from the other. Having the image disparity as well as the baseline distance between the cameras and the camera’s focal length, depth map of the image can be predicted. Despite offering some promising results, this method has some limitations such as generating inconsistent depth information on specular and transparent surfaces as well as creating artifacts at occlusion boundaries as a result of some pixels being invisible in one of the stereo images.

  \item \textbf{Unsupervised CNN for Single View Depth Estimation: Geometry to the Rescue}\\ 
Garg et al. \cite{Garg2016Unsupervised} train the network using pairs of images with a known camera motion between them. This method makes use of stereo pairs, however, it can also be similarly applied to the data generated from a moving Simultaneous Localization and Mapping (SLAM) system. Such data is more easily acquired than ground truth depth maps. The non-linear transformation which transforms an image to a depth-map is modeled through a CNN. The loss function that is utilized to train this CNN is the photometric difference between the source image (one pair of the stereo images) and the inverse-warped target image (the other stereo pair) which is both differentiable and correlated with prediction error. This approach was presented as an alternative to training on massive ground truth depth maps. However, stereo images are not always part of the target dataset while ground truth depth maps might be.

  \item \textbf{A Large RGB-D Dataset for Semi-supervised Monocular Depth Estimation \cite{Cho2019Large}}\\
In this paper, a semi-supervised approach based on the student-teacher strategy \cite{Xu} is utilized. The teacher network uses a massive unlabeled stereo image dataset as an input. Using off-the-shelf stereo matching \cite{Pang2017Cascade} CNN trained with ground truth depth data, depth maps of the images are created. To improve performance and compensate for some limitations that this model might have, such as poor estimation due to occlusion, poor illumination and specular surfaces, stereo confidence maps \cite{Park2015Leveraging} are used as an auxiliary data. These confidence maps are also used in the student network to avoid utilization of inaccurate stereo depth values. Finally, outputted depth maps and stereo confidence maps are used as pseudo ground truth to supervise the monocular student network. This approach has been tested on multiple datasets and is free of model adaptation issues as a result of utilizing pseudo depth maps through a student-teacher strategy. The overall framework is illustrated in Figure~\ref{figure:1}.

\begin{figure}[H!]
  \centering
  %\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \includegraphics[scale=0.55]{Fig1.png}
  \caption{First step is to generate depth maps from stereo image pairs using deep teacher network trained with ground truth depth data. The stereo confidence map is also estimated to recognize inaccurate depth values. Then, the monocular student network is trained with the output of the teacher network, pseudo ground truth depth maps and stereo confidence maps. Reprinted from \cite{Cho2019Large}}
  \label{figure:1}
\end{figure}


\end{itemize}

\subsection{Supervised approaches}
In supervised learning algorithms, the model is trained on pixel-level ground truth depth values. Some methods use partial depth maps in training phase, and as a result, different requirements and constraints need to be introduced to achieve better performance.
\begin{itemize}
  \item \textbf{Depth Map Prediction from a Single Image using a Multi-Scale Deep Network \cite{Eigen2014Depth}}\\
Ground truth depth information of RGB images is obtained from Kinect or laser data for training, however, during inference, depth is estimated only using the RGB images. The main idea of this method is to achieve better performance by utilizing information obtained from both global and local views. The neural network contains two components: one for estimating the global structure of the scene, and a second that refines the first one by utilizing local information. The loss function explicitly accounts for depth relations between pixel locations as well as the pointwise error. This approach has been tested on NYU Depth and KITTI \cite{Geiger2012Are} datasets and has achieved better performance compared to Make3D \cite{Saxena2007Learning}, as well as Karsch et al \cite{Karsch2014Depth} and Ladicky et al \cite{Ladický2014Pulling} methods. 

\item \textbf{Deep Ordinal Regression Network for Monocular Depth Estimation \cite{Fu2018Deep}}\\
This approach phrases the problem as an ordinal regression task instead of a continuous depth map prediction and quantizes the outputs to intervals. Continuous depth maps are discretized into a number of intervals using a space-increasing discretization (SID) strategy that allows a relatively large error when predicting larger depth values to avoid over-strengthened influence of large depth values in the training phase. Although one approach is to pass discretized depth values to a multi-class classifier, but this would lose the importance of ordering. Therefore, the problem is casted as an ordinal regression problem. The network architecture is divided into two sections: a feature extractor and a scene understanding module to capture global contextual information. Training a regression network is slow in convergence and might result in underfitting. Using ordinal regression method instead, elevates the overall performance.

\item \textbf{MultiDepth: Single-Image Depth Estimation via Multi-Task Regression and Classification \cite{Liebel2019MultiDepth:}}\\
MultiDepth takes the novel MTL approach to monocular depth estimation to overcome the instability and slow convergence of depth estimation during supervised training. It uses depth interval classification as an auxiliary task during training phase and at inference, it only predicts continuous depth values by disabling the use of that auxiliary task. This approach has been tested on the KITTI dataset for road scenes. The ground truth depth information obtained from LiDAR sensors are used as the training data for the main regression task. They are also classified into a number of intervals to be used as the auxiliary task and improve the performance of single image depth estimation. 

\item \textbf{Estimated Depth Map Helps Image Classification\cite{He2017Estimated}}\\
This paper investigates the effect of including estimated depth maps as an extra channel to the network and if it can improve the image classification task. To achieve this, they first estimate depth maps for the CIFAR-10 RGB images using a trained deep convolutional neural field model. Then, depth maps are added as a new channel along with RGB images to build a RGBD dataset. Finally, the newly created RGBD dataset is used as an input to the image classifier to detect which category they belong to out of the original 10 classes. Using this technique, the accuracy was improved by 0.55\% in ResNet-20.

\end{itemize}

\section{Datasets}
Classification is a popular topic in computer vision where we want to either classify images based on their overall theme or classify objects in images to improve image understanding and analysis. There are numerous datasets which are formed for the task of classification. In contrast, depth estimation demands complex ground truths of depth maps, and thus dataset options are limited. We worked on two different paradigms: customized MNIST-based datasets and NYU Depth V2

\subsection{MNIST}
MNIST is a dataset of handwritten digits, commonly used in classification problems. MNIST exists in multiple formats, such as Numpy, Pickle, and even in the form of tabular data, and is included in different libraries. We created a series of customized MNIST based datasets by introducing noise to specific images and resizing them. We chose to work with the original MNIST because we aimed for maximum level of control and insight over the dataset. Originally, MNIST images have the fixed size of 28x28. There are 60,000 and 10,000 images in train and test cohorts, respectively. To approach real-world images, we upsample each image to 256x256. For our experiments, we had to create depth maps for the images. To normalize the dataset, we first divide the array of each image by 255 which is the maximum pixel value of MNIST (or any other grayscale dataset). Then we binarize images using the threshold of 0.5. The resulting black and white numbers are extruded with a fixed depth which is proportional to their class value, as is depicted in Figure~\ref{figure:2}. On the other hand, we manipulate the dataset through two mechanisms: dataset size (examples included) and adding noise to images.
\begin{figure}[H!]
  \centering
  %\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \includegraphics[scale=0.55]{Fig2.png}
  \caption{Illustration of our extruded MNIST}
  \label{figure:2}
\end{figure}

\subsection{NYU Depth V2}
NYU-Depth-V2 dataset includes RGB and depth images of indoor scenes along with segmentation and classification of objects inside each image. This dataset can be a good choice for the semantic segmentation of the images. However, we found out the classification labels classify objects into structural classes that reflect their physical role in the scene, thus they are not appropriate for conventional classification purposes such as scene classification. Therefore, we manually labeled the dataset for scene classification task.
Kitchen: 0
Office: 1
Classroom: 2
Living Room: 3
Washroom: 4
Bedroom: 5
Store: 6



total:1449
0: 208
1:199
2:80
3: 438
4: 127
5: 330
6: 67


Another technical problem of the NYU-Depth dataset is its format. It was created to be used within MATLAB. Nonetheless, using existing Python libraries, we managed to load the dataset and access its low-level properties. We have made our preprocessed NYU dataset public and all the manual labels along with notes and instructions are available. 

\section{Model Architecture}
The main goal of this research is training a network for the depth regression and classification tasks to share parameters and enforce the learning of a common representation. Our network is given an image of a scene and produces two different outputs: depth map and class label. Depth maps contain the pixel-level depth information of the image, while class labels include the predicted class that the image belongs to. The fact that we aim to output depth maps implies that the Fully Convolutional Networks (FCNs) are appropriate candidates for our purpose. Therefore, we opt U-Net \cite{Ronneberger0U-Net:}, which is the core of state-of-the-art approaches for segmentation tasks and benchmark of depth estimation \cite{Cho2019Large}, to act as the backbone of our model. In order to produce the classification output, we utilize the feature flow at the bottleneck of our U-Net.
Our network simply generalizes U-Net to joint depth regression and classification tasks. U-net outputs a single depth map while we add a parallel branch that extracts features for the classification task and outputs the class label. The U-Net is composed of two sub-networks: encoding and decoding networks. The encoding network includes encoding blocks to learn input representations, and down sampling blocks to encode the input image at multiple levels into feature representations. In our experiments, this part is shared between the depth estimator and the classifier. The goal of the decoding network is to restore features learnt by the encoder onto the higher resolution space similar to the original image. In our architecture, this part is depth-estimator-specific. U-Net also contains skip connections to enable encoder and decoder to share information. The parallel branch we add to the U-Net structure for classification purpose, uses the same encoder structure of the depth estimator U-Net, while in second stage, it adds a branch with fully connected layers to output classification labels. The full model architecture and details of each block of the network are indicated in Figures~\ref{figure:3} and~\ref{figure:4}.

\begin{figure}[h!]
  \centering
  %\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \includegraphics[scale=0.50]{Fig3.png}
  \caption{Model Architecture}
  \label{figure:3}
\end{figure}

\begin{figure}[h!]
  \centering
  %\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \includegraphics[scale=0.7]{Fig4.png}
  \caption{Model parts}
  \label{figure:4}
\end{figure}


\section{Experiments}
Our experiments consist of three main parts. First, different amounts of noise were added to the input image and the accuracy of classification was calculated. Then we created images similar to depth maps for each image and used them to train a depth estimator along with our classification using dMTL approach. This approach robustly improved the classification performance. Next, the number of training images was manipulated and same approach as above was tested on each new dataset. Finally, we examined effect of different dMTL training methods to determine the best optimization method.

Throughout our experiments with MNIST we used a fixed set of hyperparameters. Our learning rate was \( 5\times10^{-5} \), L2 penalty was 0.001, momentum was chosen to be 0.9, batch size was equal to 4, we limited our experiments to 10 epochs, and we used weighted Cross Entropy (CE) as our loss function for the classification task. Given the fact that our dataset was almost balanced, unweighted CE would create same results. We used the first N examples of the MNIST training cohort for training. 1500 examples (index 45000 to 46500) from the MNIST training cohort formed our validation set and the first 1000 examples of the MNIST test set were used as our test cohort.

Table~\ref{table:1} and Figure~\ref{figure:5} show results of experiments using 5000 training examples. As anticipated, higher levels of noise associate with lower performance of the model for both depth estimation and classification tasks. Worthy to be highlighted, the model maintains most of its test accuracy in highly noisy environments, but depth estimation results are degraded. Although dMTL elevates classification performance at different noise levels, the test accuracy improvements are not considerable.

\begin{table}
  \caption{Performance of the depth estimation model at different SNRs, with N=5000, with dMTL}
  \label{table:1}
  \centering
  \resizebox{\textwidth}{!}{\begin{tabular}{llllll}
    S:N&	N&	Test Accuracy&	Input&	Depth Estimation Output&	Ground Truth Depth Map\\
    \midrule
    Inf&	5000&	0.967&  
    \begin{minipage}{.3\textwidth}
      \includegraphics[width=\linewidth, height=\imgdim, width=\imgdim]{images/img1.PNG}
    \end{minipage}&
    \begin{minipage}{.3\textwidth}
      \includegraphics[width=\linewidth, height=\imgdim, width=\imgdim]{images/img2.PNG}
    \end{minipage}&
    \begin{minipage}{.3\textwidth}
      \includegraphics[width=\linewidth, height=\imgdim, width=\imgdim]{images/img3.PNG}
    \end{minipage}\\
    \midrule
    1:5&	5000&	0.953&
    \begin{minipage}{.3\textwidth}
      \includegraphics[width=\linewidth, height=\imgdim, width=\imgdim]{images/img4.PNG}
    \end{minipage}&
    \begin{minipage}{.3\textwidth}
      \includegraphics[width=\linewidth, height=\imgdim, width=\imgdim]{images/img5.PNG}
    \end{minipage}&
    \begin{minipage}{.3\textwidth}
      \includegraphics[width=\linewidth, height=\imgdim, width=\imgdim]{images/img6.PNG}
    \end{minipage}\\
    \midrule
    1:19&	5000&	0.912&
    \begin{minipage}{.3\textwidth}
      \includegraphics[width=\linewidth, height=\imgdim, width=\imgdim]{images/img7.PNG}
    \end{minipage}&
    \begin{minipage}{.3\textwidth}
      \includegraphics[width=\linewidth, height=\imgdim, width=\imgdim]{images/img8.PNG}
    \end{minipage}&
    \begin{minipage}{.3\textwidth}
      \includegraphics[width=\linewidth, height=\imgdim, width=\imgdim]{images/img9.PNG}
    \end{minipage}\\
    \midrule
    1:29&	5000&	0.851&
    \begin{minipage}{.3\textwidth}
      \includegraphics[width=\linewidth, height=\imgdim, width=\imgdim]{images/img10.PNG}
    \end{minipage}&
    \begin{minipage}{.3\textwidth}
      \includegraphics[width=\linewidth, height=\imgdim, width=\imgdim]{images/img11.PNG}
    \end{minipage}&
    \begin{minipage}{.3\textwidth}
      \includegraphics[width=\linewidth, height=\imgdim, width=\imgdim]{images/img12.PNG}
    \end{minipage}\\
    \bottomrule
  \end{tabular}}
\end{table}









no noise classes: 0 and 1 kitchen-classroom
mtloss 2cls: val: 0.6774193548387096, test0.5918367346938775
cls only 2cls: val:0.6935483870967742 , test 0.6122448979591837
---
no noise classes: 0 and 2 kitchen-classroom
mtloss 2cls: val: 70, test76
cls only 2cls: val:66 , test 72
---
no noise classes: 0 and 3 kitchen-livingroom
mtloss 2cls: 0.8144329896907216val: , 0.7448979591836735test
cls only 2cls: 0.7938144329896907 val: , 0.7755102040816326test
---
no noise classes: 0 and 4 kitchen-washroom
mtloss 2cls: val: 0.8431372549019608 , test0.7560975609756098
cls only 2cls: val: 0.8235294117647058, test0.8048780487804879
---
no noise classes: 0 and 6 kitchen-store
mtloss 2cls: val:0.8536585365853658 , test0.8780487804878049
cls only 2cls: val:0.8292682926829268 , test0.8048780487804879
--
no noise classes: 0 and 5
mtloss 2cls: val: 85 , test 89
cls only 2cls: val:80 , test82
--
no noise classes: 0 and 5 vs 6
mtloss 2cls: val: 0.7920792079207921 , test 0.8282828282828283
cls only 2cls: val:0.7623762376237624 , test0.6363636363636364
---
no noise classes: 0 and 3vs 5 vs 6
mtloss 2cls: val: 0.5705882352941176, test 0.5595238095238095
cls only 2cls: val:0.5352941176470588 , test0.5357142857142857
---
no noise classes: 0 and 4vs 5 vs 6
mtloss 2cls: val: 0.7338709677419355, test 0.7657657657657657
cls only 2cls: val:0.6612903225806451 , test0.6666666666666666

\section{Conclusion}
We presented a method for improving performance of deep models in presence of noise and when the dataset size is limited. In extensive experiments, we showed the how classification and depth estimation tasks can act as complementary operations. We also explored all multitasking approached for training our deep model. Our experiments revealed multitask loss is the most effective method.
\end{comment}
